AtlasNet: A Papier-M\^ach\'e Approach to Learning 3D Surface Generation

We introduce a method for learning to generate the surface of 3D shapes. Our approach represents a 3D shape as a collection of parametric surface elements and, in contrast to methods generating voxel grids or point clouds, naturally infers a surface representation of the shape. Beyond its novelty, our new shape generation framework, AtlasNet, comes with significant advantages, such as improved precision and generalization capabilities, and the possibility to generate a shape of arbitrary resolution without memory issues. We demonstrate these benefits and compare to strong baselines on the ShapeNet benchmark for two applications: (i) auto-encoding shapes, and (ii) single-view reconstruction from a still image. We also provide results showing its potential for other applications, such as morphing, parametrization, super-resolution, matching, and co-segmentation.

==> content/CVPRStyleGuide.tex <==

Please follow the steps outlined below when submitting your manuscript to
the IEEE Computer Society Press.  This style guide now has several
important modifications (for example, you are no longer warned against the
use of sticky tape to attach your artwork to the paper), so all authors
should read this new version.

%
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the CVPR 2018 web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section,
must be no longer than eight pages in length. The references section
will not be included in the page count, and there is no limit on the
length of the references section. For example, a paper of eight pages
with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for CVPR 2018.}

Overlength papers will simply not be reviewed.  This includes papers
where the margins and formatting are deemed to have been significantly
altered from those laid down by this style guide.  Note that this
\LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for
supervised revisions of manuscripts.  The reviewing process cannot determine
the suitability of the paper for presentation in eight pages if it is
reviewed in eleven.  

%
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document using a non-\LaTeX\
document preparation system, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. (\LaTeX\ users may uncomment
the \verb'\cvprfinalcopy' command in the document preamble.)  Reviewers:
note that the ruler measurements do not align well with lines in the paper
--- this turns out to be very difficult to do well when the paper contains
many figures and equations, and, when done, looks ugly.  Just use fractional
references (e.g.\ this line is $095.5$), although in most cases one would
expect that the approximate location will be adequate.

\subsection{Mathematics}

Please number all of your sections and displayed equations.  It is
important for readers to be able to refer to any particular equation.  Just
because you didn't refer to it in the text doesn't mean some future reader
might not need to refer to it.  It is cumbersome to have to use
circumlocutions like ``the equation second from the top of page 3 column
1''.  (Note that the ruler will not be present in the final copy, so is not
an alternative to equation numbers).  All authors will benefit from reading
Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.


\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind
review.  Blind review does not mean that one must remove
citations to one's own work---in fact it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  That is all.  (But see below for
techreports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith; it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith \etal [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time,
which covers similar or overlapping material, you may need to refer to that
submission in order to explain the differences, just as you would if you
had previously published related work.  In such cases, include the
anonymized parallel submission~\cite{Authors14} as additional material and
cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324,
Supplied as additional material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be
found elsewhere, and refer them to a technical report.  For conference
submissions, the paper must stand on its own, and not {\em require} the
reviewer to go to a techreport for further details.  Thus, you may say in
the body of the paper ``further details may be found
in~\cite{Authors14b}''.  Then submit the techreport as additional material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the CVPR70 audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention,
reads better than the first version, and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B.

FAQ: Are acknowledgements OK?  No.  Leave them for the final copy.


\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %
\end{center}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``
   Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
\cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

%
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.



%
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.


%
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors14}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

%
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths which render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}


%
\subsection{Color}

Please refer to the author guidelines on the CVPR 2018 web page for a discussion
of the use of color in your document.

%
\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.

Please direct any questions to the production editor in charge of these
proceedings at the IEEE Computer Society Press: Phone (714) 821-8380, or
Fax (714) 761-1784.

{\small
\bibliographystyle{ieee}
\bibliography{egbib}
}


==> content/conclusion_future_work.tex <==
We have introduced an approach to generate parametric surface elements for 3D shapes. 
We have shown its benefits for 3D shape and single-view reconstruction, out-performing existing baselines. 
In addition, we have shown its promises for shape interpolation, finding shape correspondences, and mesh parameterization. 
Our approach opens up applications in generation and synthesis of meshes for 3D shapes, similar to still image generation~\cite{Isola:2017,Zhu:2017:cylcegan}.



==> content/introduction-nov13.tex <==



   

%
%

%
%
%
%

Huge progresses have been made on learning good representations for images, allowing impressive applications in particular for image generation~\cite{Isola:2017,Zhu:2017:cylcegan}. On the contrary, the challenge of learning good representations for 3D shapes remains widely open. 
Recent work have considered training convolutional neural network on meshes \cite{Masci15,Boscaini16,bronstein2017geometric}, leveraging or generating volumetric \cite{choy20163d,TDB17b,Hane:2017} or point cloud \cite{qi2016pointnet,Fan:2017:cvpr,Qi:2017:nips} representations of 3D shape, without one representations reaching consensus or obtaining fully satisfactory results. In this work, inspired by the topological definition of a surface, as being everywhere similar to the Euclidean plane, we explore a different type of representation for high quality surface generation. As visualized in the teaser, we learn to generate surfaces by representing them as the image of a set of \patches. \\ %

%
This is especially true for the most common shape representation used in computer graphics and robotics: a surface. 
%
%
%
%

%
%
%


%
\mathieu{I liked having the question 'Why learning to generate surfaces?', but couldn't make it work with the text flow: if you have an idea, feel free.}
%
%
Having such a representation of a shape surface is extremely valuable, since it allows to easily represent its properties, such as its texture and physical properties, via a mapping to a texture atlas.%
The ability to learn to generate such a representation would allow applications in rendering for computer graphics, and interaction and manipulation for robotics. 

Another important advantage of our approach is that it allows to naturally generate a regular mesh of the reconstructed surface. Meshes are indeed a simple and compact representation of a shape, which makes them %
%
%
%
%
%
The ability to {learn} to generate 3D surfaces would enable applications in computer assisted design. The artistic design of triangle meshes is indeed a significant portion of the cost of creating 3D content, but current generative methods for 3D surfaces often suffer from the issue that the mesh representation does not trivially map to a regular structure. Instead, generative methods for surfaces typically  %


\begin{figure}[t!]
\centering
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{}
\caption{Possible inputs}
\end{subfigure}
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{}
\caption{Raw output}
\end{subfigure}
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{}
\caption{Optimized atlas}
\end{subfigure}
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{}
\caption{Optimized mesh}
\end{subfigure}
\caption{{\bf \ournet }
}
  \label{fig:teaser}
\end{figure}
   



\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{figures/overview/baselineb.pdf}
\caption{Baseline. \label{fig:baseline}}
\end{subfigure}
~\vline~
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{figures/overview/ours_1b.pdf}
\caption{Our approach with one patch. \label{fig:ours1}}
\end{subfigure}
~\vline~
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{figures/overview/ours_Kc.pdf}
\caption{Our approach with K patches. \label{fig:oursK}}
\end{subfigure}
\caption{{\bf Overview of our approach.} We focus on architectures for shape generation. We thus take as input a latent shape representation (that can be learned jointly with a reconstruction objective) and generate as output a set of points. (\ref{fig:baseline}) A baseline deep architecture would simply decode this latent representation into a set of points of a given size. (\ref{fig:ours1}) On the contrary, our approach  takes as additional input a 2D point sampled uniformly in the unit square and use it to generate a single point. Our output is thus the continuous image of a planar surface, from which the topology can easily be transferred. In particular, we can easily infer a mesh, with any resolution, on the generated surface elements. (\ref{fig:ours1}) This strategy can easily be repeated multiple times  to represent a 3D shape as the union of several surface elements.
}
  \label{fig:overview}
\end{figure*}


\paragraph{Challenges.} %
Generating the mesh of a surface is a difficult problem. Indeed, generating a mesh directly would require to infer both the 3D position of the vertices and the triangles connecting them. An alternative approach is to use another representation of the 3D shape, such as a point cloud or a voxel grid, then used specialized techniques to convert this representation into a triangle mesh. Generating high-resolution meshes with sharp features thus requires that special care be taken to mitigate undesirable effects of this conversion between the underlying representation and a triangle mesh, a difficulty that would be avoided by a method directly generating meshes.\\



To address these challenges, we propose to interpret both the feature representation of a shape as parameters for local parametric representations of the surface. These parameters are used by generation networks to build local map between the 2D Euclidean square and the surface of the 3D shape. Our representation of a shape is thus extremely similar to an atlas, as we will discuss in section \ref{sec:theory}. Sampling points on the unit square allows us to generate any number of points on the surface, but we can also transfer richer data, such as a regular mesh, from the 2D square to our generated shape.\\


Since it deforms primitive surface elements into a 3D shape, our work can be seen as bridging the gap between the recent works that learn to represent 3D shapes as a set of simple primitives, with a fixed, low number of parameters \cite{tulsiani2016learning} and those that represent 3D shapes as an unstructured set of points ~\cite{Fan:2017:cvpr}. It can also be interpreted as learning as a factored representation of a surface, where a point on the shape is represented jointly by a vector encoding the shape structure and a vector encoding its position. Finally, it can be seen as an attempt to bring to 3D the power of convolutional approaches for generating 2D images~\cite{Isola:2017,Zhu:2017:cylcegan} by sharing the network parameters for parts of the surface.


\paragraph{Our contributions.} 
In this paper:
\begin{itemize}
    \item we propose a novel approach to 3D meshes generation, dubbed {\it \ournet}, which is composed of a union of \patches. These \patches are parametric transformations of a set of 2D rectangles tothe surface, covering it in a way similar to placing strips of paper on a shape to form a papier-m\^ach\'e. The parameters of the transformations come both from the learned weights of a neural network and a learned representation of the shape. 
    \item We show that the learned parametric transformation maps locally everywhere to a surface, naturally adapt to its underlying complexity, can be sampled at any desired resolution and allows for transfer of a tessellation or texture map to the generated surface. 
    \item We demonstrate the advantages of our approach both qualitatively and quantitatively on surface generation form (potentially low resolution) point clouds and 2D images
    \item we demonstrate the potential of our method for several applications, including shape interpolation, parameterization, and shape collections alignment. 
   
\end{itemize}
%



==> content/introduction.tex <==
\vspace{-2mm}
Significant progress has been made on learning good representations for images, allowing impressive applications in image generation~\cite{Isola:2017,Zhu:2017:cylcegan}. However, learning a representation for generating high-resolution 3D shapes remains an open challenge. Representing a shape as a volumetric function~\cite{choy20163d,Hane:2017,TDB17b} only provides voxel-scale sampling of the underlying smooth and continuous surface. In contrast, a point cloud~\cite{qi2016pointnet,Qi:2017:nips} provides a representation for generating on-surface details~\cite{Fan:2017:cvpr}, efficiently leveraging sparsity of the data. However, points do not directly represent neighborhood information, making it difficult to approximate the smooth low-dimensional manifold structure with high fidelity. 

To remedy shortcomings of these representations, surfaces are a popular choice in geometric modeling. A surface is commonly modeled by a  polygonal mesh: a set of vertices, and a list of triangular or quad primitives composed of these vertices, providing piecewise planar approximation to the smooth manifold. Each mesh vertex contains a 3D (XYZ) coordinate, and, frequently, a 2D (UV) embedding to a plane. The UV parameterization of the surface provides an effective way to store and sample functions on surfaces, such as normals, additional geometric details, textures, and other reflective properties such as BRDF and ambient occlusion. 
One can imagine converting point clouds or volumetric functions produced with existing learned generative models as a simple post-process. %
However, this requires solving two fundamental, difficult, and long-standing challenges in geometry processing: global surface parameterization and meshing. 

%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{figures/overview/baselineb.pdf}
\caption{Points baseline. \label{fig:baseline}}
\end{subfigure}
~\vline~
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{figures/overview/ours_1b.pdf}
\caption{Our approach with one patch. \label{fig:ours1}}
\end{subfigure}
~\vline~
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{figures/overview/ours_Kc.pdf}
\caption{Our approach with K patches. \label{fig:oursK}}
\end{subfigure}
\caption{{\bf Shape generation approaches.} All methods take as input a latent shape representation (that can be learned jointly with a reconstruction objective) and generate as output a set of points. (a) A baseline deep architecture would simply decode this latent representation into a set of points of a given size. (b) Our approach takes as additional input a 2D point sampled uniformly in the unit square and uses it to generate a single point on the surface. Our output is thus the continuous image of a planar surface. In particular, we can easily infer a mesh of arbitrary resolution on the generated surface elements. (c) This strategy can be repeated multiple times to represent a 3D shape as the union of several surface elements.
}
  \label{fig:overview}
  \vspace*{-4mm}
\end{figure*}


In this paper we explore learning the surface representation directly.  Inspired by the formal definition of a surface as a topological space that locally resembles the Euclidean plane, we seek to approximate the target surface locally by mapping a set of squares to the surface of the 3D shape. The use of multiple such squares allows us to model complex surfaces with non-disk topology. Our representation of a shape is thus extremely similar to an atlas, as we will discuss in Section \ref{sec:theory}. The key strength of our method is that it jointly learns a parameterization and an embedding of a shape. This helps in two directions. First, by ensuring that our 3D points come from 2D squares we favor learning a continuous and smooth 2-manifold structure. Second, by generating a UV parameterization for each 3D point, we generate a global surface parameterization, which is key to many applications such as texture mapping and surface meshing. Indeed, to generate the mesh, we simply transfer a regular mesh from our 2D squares to the 3D surface, and to generate a regular texture atlas, we simply optimize the metric of the square to become as-isometric-as-possible to the corresponding 3D shape (Fig.~\ref{fig:teaser_fig}). 

Since our work deforms primitive surface elements into a 3D shape, it can be seen as bridging the gap between the recent works that learn to represent 3D shapes as a set of simple primitives, with a fixed, low number of parameters \cite{tulsiani2016learning} and those that represent 3D shapes as an unstructured set of points~\cite{Fan:2017:cvpr}. It can also be interpreted as learning a factored representation of a surface, where a point on the shape is represented jointly by a vector encoding the shape structure and a vector encoding its position. Finally, it can be seen as an attempt to bring to 3D the power of convolutional approaches for generating 2D images~\cite{Isola:2017,Zhu:2017:cylcegan} by sharing the network parameters for parts of the surface.

%

\myparagraph{Our contributions.} 
In this paper:
\begin{itemize}
  \vspace*{-1mm}
    \item We propose a novel approach to 3D surface generation, dubbed {\it \ournet}, which is composed of a union of \patches. These \patches~transform a set of 2D squares to the surface, covering it in a way similar to placing strips of paper on a shape to form a papier-m\^ach\'e. The parameters of the transformations come both from the learned weights of a neural network and a learned representation of the shape. 
      \vspace*{-1mm}
    \item We show that the learned parametric transformation maps locally everywhere to a surface, naturally adapts to its underlying complexity, can be sampled at any desired resolution, and allows for the transfer of a tessellation or texture map to the generated surface. 
      \vspace*{-1mm}
    \item We demonstrate the advantages of our approach both qualitatively and quantitatively on high resolution surface generation from (potentially low resolution) point clouds and 2D images
      \vspace*{-1mm}
    \item We demonstrate the potential of our method for several applications, including shape interpolation, parameterization, and shape collections alignment. 
\end{itemize}
All the code is available at the project webpage\footnote{\url{https://github.com/ThibaultGROUEIX/AtlasNet}.}. 


==> content/method.tex <==
\section{\ournet}
\label{sec:implementation}

In this section we introduce our model, \ournet{}, which decodes a 3D surface given an encoding of a 3D shape. This encoding can come from many different representations such as a point cloud or an image (see Figure~\ref{fig:teaser_fig} for examples).

%



\newcommand{\groundtruth}{\mathcal{S}^\star}
\newcommand{\patchinput}{\mathcal{A}}
\newcommand{\shapefeature}{\mathbf{x}}
\newcommand{\mlp}{\varphi}
\newcommand{\lossmlp}{\mathcal{L}}
\newcommand{\lossatlas}{\mathcal{L}^\prime}
\newcommand{\parameters}{\theta}
\newcommand{\parameterset}{\Theta}


\subsection{Learning to decode a surface}

Our goal is, given a feature representation $\shapefeature$ for a 3D shape, to generate the surface of the shape. 
As shown in Section~\ref{sec:theory}, an MLP with ReLUs $\mlp_\parameters$ with parameters $\parameters$ can locally generate a surface by learning to map points in $\mathbb{R}^2$ to surface points in $\mathbb{R}^3$. To generate a given surface, we need several of these learnable charts to represent a surface. In practice, we consider $N$ learnable parameterizations $\phi_{\theta_i}$ for $i \in \lbrace 1,\ ...,N\rbrace$.
To train the MLP parameters $\theta_i$, we need to address two questions: (i) how to define the distance between the generated and target surface, and (ii) how to account for the shape feature $\shapefeature$ in the MLP?
%
%
%
%
To represent the target surface, we use the fact that, independent of the representation that is available to us, we can sample points on it. Let $\patchinput$ be a set of points sampled in the unit square $[0,1]^2$ and $\groundtruth$  a set of points sampled on the target surface.
Next, we incorporate the shape feature $\shapefeature$ by simply concatenating them with the sampled point coordinates $\mathbf{p}\in\patchinput$ before passing them as input to the MLPs. 
%
Our model is illustrated in Figure~\ref{fig:ours1}. Notice that the MLPs are not explicitly prevented from encoding the same area of space, but their union should cover the full shape. Our MLPs do depend on the random initialization, but similar to convolutional filter weights the network learns to specialize to different regions %
in the output without explicit biases.
We then minimize the Chamfer loss between the set of generated 3D points and $\groundtruth$,
%
\begin{multline}
    \lossmlp(\parameters) = \sum_{\mathbf{p}\in\patchinput}\sum_{i=1}^N  \min_{\mathbf{q}\in\groundtruth} \left|\phi_{\theta_i}\left(\mathbf{p}; \shapefeature\right) - \mathbf{q}\right|^2\\
    + \sum_{\mathbf{q}\in\groundtruth}  \min_{i \in \lbrace 1,\ ...,N\rbrace}\min_{\mathbf{p}\in\patchinput}\left|\phi_{\theta_i}\left(\mathbf{p}; \shapefeature\right) - \mathbf{q}\right|^2.
\label{eqn:atlas_loss}
\end{multline}
%

%

%
%
%
%
%
%
%
%

%

%


\subsection{Implementation details}

%

We consider two tasks: (i) to auto-encode a 3D shape given an input 3D point cloud, and (ii) to reconstruct a 3D shape given an input RGB image. For the auto-encoder, we used an encoder based on PointNet~\cite{qi2016pointnet}, which has proven to be state of the art on point cloud analysis on ShapeNet and ModelNet40 benchmarks. 
This encoder transforms an input point cloud into a latent vector of dimension $k=1024$. We experimented with input point clouds of 250 to 2500 points. For images, we used ResNet-18 \cite{he2016deep} as our encoder. The architecture of our decoder is 4 fully-connected layers of size 1024, 512, 256, 128 with ReLU non-linearities on the first three layers and tanh on the final output layer. We always train with output point clouds of size 2500 evenly sampled across all of the learned parameterizations -- scaling above this size is time-consuming because our implementation of Chamfer loss has a compute cost that is quadratic in the number of input points. 
We experimented with different basic weight regularization options but did not notice any generalization improvement.
%
%
%
Sampling of the learned parameterizations as well as the ground truth point-clouds is repeated at each training step to avoid over-fitting. To train for single-view reconstruction, we obtained the best results by training the encoder and using the decoder from the point cloud autoencoder with fixed parameters.
Finally, we noticed that sampling points regularly on a grid on the learned parameterization yields better performance than sampling points randomly. All results used this regular sampling.

%


%

\subsection{Mesh generation}
\label{sec:mesh}
The main advantage of our approach is that during inference, we can easily generate a mesh of the shape.


\myparagraph{Propagate the patch-grid edges to the 3D points.} 
The simplest way to generate a mesh of the surface is to transfer a regular mesh on the unit square to 3D, connecting in 3D the images of the points that are connected in 2D. Note that our method allows us to generate such meshes at very high resolution, without facing memory issues, since the points can be processed in batches. We typically use 22500 points. As shown in the results section, such meshes are satisfying, but they can have several drawbacks: they will not be closed, may have small holes between the images of different learned parameterizations, and different patches may overlap. %
%

\myparagraph{Generate a highly dense point cloud and use Poisson surface reconstruction (PSR) ~\cite{kazhdan2013screened}.}
To avoid the previously mentioned drawbacks, we can additionally densely sample the surface and use a mesh reconstruction algorithm. We start by generating a surface at a high resolution, as explained above. We then shoot rays at the model from infinity and obtain approximately 100000 points, together with their oriented normals, and then can use a standard oriented cloud reconstruction algorithm such as PSR to produce a triangle mesh. We found that high quality normals as well as high density point clouds are critical to the success of PSR, which are naturally obtained using this method. %

\myparagraph{Sample points on a closed surface rather than patches.} To obtain a closed mesh directly from our method, without requiring the PSR step described above, we can sample the input points from the surface of a 3D sphere instead of a 2D square. The quality of this method depends on how well the underlying surface can be represented by a sphere, which we will explore in Section~\ref{sec:autoencoding}. 

%

%
%
%



==> content/proof.tex <==
\section{Proof (to be included in supp. material)}

\begin{proof}
The gist of the proof is the MLP is continuous, and different settings of the ReLUs generates a polygonal tessellation of $A$. 
The MLP linearly maps each interior polygonal point, and we can define an open set (either open interval or open disc) around each of these points such that the MLP is a homeomorphism. 
All other points in $A$ are boundary points, and we have to show that, for each boundary point, we can find a set containing the boundary point such that there is a homeomorphism to a half interval or half disc, and that the MLP is a homeomorphism over the set. 
\end{proof}


==> content/related_work.tex <==
\section{Related work}
\label{sec:related}

%
3D shape analysis and generation has a long history in computer vision. In this section, we only discuss the most directly related works for representation learning for 2-manifolds and 3D shape generation using deep networks.
%
%
\myparagraph{Learning representations for 2-manifolds.}
A polygon mesh is a widely-used representation for the 2-manifold surface of 3D shapes.
Establishing a connection between the surface of the 3D shape and a 2D domain, or surface parameterization, 
is a long-standing problem in geometry processing, 
with applications in texture mapping, re-meshing, and shape correspondence~\cite{Hormann08}.
Various related representations have been used for applying neural networks on surfaces. 
The geometry image representation~\cite{Gu02,Sander03} views 3D shapes as functions (e.g., vertex positions) 
embedded in a 2D domain, providing a natural input for 2D neural networks~\cite{Sinha2016}. 
Various other parameterization techniques, such as local polar 
coordinates~\cite{Masci15,Boscaini16} and global seamless maps~\cite{Maron17}
have been used for deep learning on 2-manifolds. 
%
%
%
%
%
%
%
Unlike these methods, we do not need our input data to be parameterized. Instead, we learn 
the parameterization directly from point clouds. Moreover, these methods assume that the training and testing data are 2-manifold meshes, and thus cannot easily be used for surface reconstructions from point clouds or images. 

%
%
%

\myparagraph{Deep 3D shape generation.} 
%
%
Non-parametric approaches retrieve shapes from a large corpus~\cite{Bansal:2016,Li:2015:purification,Massa:2016}, but require having an exact instance in the corpus. 
One of the most popular shape representation for generation is the voxel representation. %
%
Methods for generating a voxel grid have been demonstrated with various inputs, namely one or several images~\cite{choy20163d,Girdhar16b}, full 3D objects in the form of voxel grids \cite{Girdhar16b,wu20153d}, and 3D objects with missing shape parts~\cite{wu20153d,HRSC:2017}. 
Such direct volumetric representation is costly in term of memory and is typically limited to coarser resolutions.
To overcome this, recent work has looked at a voxel representation of the surface of a shape via oct-trees~\cite{Hane:2017,Riegler2017THREEDV,TDB17b}. Recently, Li et al. also attempted to address this issue via learning to reason over hierarchical procedural shape structures and only generating voxel representations at the part level~\cite{li_sig17}.
As an alternative to volumetric representations, another line of work has learned to encode~\cite{qi2016pointnet,Qi:2017:nips} and decode~\cite{Fan:2017:cvpr} a 3D point representation of the surface of a shape. 
A limitation of the learned 3D point representation is there is no surface connectivity (e.g., triangular surface tessellation) embedded into the representation. %

Recently, Sinha et al.~\cite{Sinha2017} proposed to use a spherical parameterization of a single deformable mesh (if available) or of a few base shapes (composed with authalic projection of a sphere to a plane) to represent training shapes as parameterized meshes. They map vertex coordinates to the resulting UV space and use 2D neural networks for surface generation. This approach relies on consistent mapping to the UV space, and thus requires automatically estimating correspondences from training shapes to the base meshes (which gets increasingly hard for heterogeneous datasets). Surfaces generated with this method are also limited to the topology and tessellation of the base mesh. Overall, learning to generate surfaces of arbitrary topology from unstructured and heterogeneous input still poses a challenge.

%
%
%
%
%
%
%

%
%
%
%
%


%
%
%
%
%
%
%
%


%






==> content/results.tex <==
In this section we show qualitative and quantitative results on the tasks of auto-encoding 3D shapes and single-view reconstruction and compare against several baselines. 
In addition to these tasks, we also demonstrate several additional applications of our approach. 
%
More results are available in the supplementary material \cite{appendix}.%

%
%
%
%
%
%
%

%
%

\myparagraph{Data.} 
We evaluated our approach on the standard ShapeNet Core dataset (v2) \cite{shapenet2015}.
%
The dataset consists of 3D models covering 13 object categories with 1K-10K shapes per category. 
We used the training and validation split provided by \cite{choy20163d} for our experiments to be comparable with previous approaches.
%
%
We used the rendered views provided by  \cite{choy20163d} and sampled 3D points on the shapes using \cite{Wang-2017-OCNN}.

\myparagraph{Evaluation criteria.}
We evaluated our generated shape outputs by comparing to ground truth shapes using two criteria. 
First, we compared point sets for the output and ground-truth shapes using Chamfer distance (``CD''). 
While this criteria compares two point sets, it does not take into account the surface/mesh connectivity. 
To account for mesh connectivity, we compared the output and ground-truth meshes using the ``Metro'' criteria using the publicly available METRO software \cite{cignoni1998metro}, which is the average Euclidean distance between the two meshes. 
%
%


\myparagraph{Points baseline.}
In addition to existing baselines, we compare our approach to the multi-layer perceptron ``Points baseline'' network shown in Figure \ref{fig:baseline}. 
%
The Points baseline network consists of four fully connected layers with output dimensions of size 1024, 512, 256, 7500 with ReLU non-linearities, batch normalization on the first three layers, and a hyperbolic-tangent non-linearity after the final fully connected layer. The network outputs 2500 3D points and has comparable number of parameters to our method with 25 learned parameterizations. The baseline architecture was designed to be as close as possible to the MLP used in \ournet{}. 
As the network outputs points and not a mesh, we also trained a second network that outputs 3D points and normals, which are then passed as inputs to Poisson surface reconstruction (PSR) ~\cite{kazhdan2013screened} to generate a mesh (``Points baseline + normals''). 
%
%
The network generates outputs in $\mathbb{R}^6$ representing both the 3D spatial position and normal. 
We optimized Chamfer loss in this six-dimensional space and normalized the normals to 0.1 length as we found this trade-off between the spatial coordinates and normals in the loss worked best. 
%
As density is crucial to PSR quality, we augmented the number of points by sampling 20 points in a small radius in the tangent plane around each point ~\cite{kazhdan2013screened}.  We noticed significant qualitative and quantitative improvements and the results shown in this paper use this augmentation scheme.
%

%
%

%


%
%
%

\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{0.12\linewidth}
\centering
 \includegraphics[height=0.6\linewidth]{figures/ae/boat_cdaff_gt_00.png}
 \includegraphics[height=0.45\linewidth]{figures/ae/avion2_GT_00.png}
 %
 \includegraphics[height=0.65\linewidth]{figures/ae/boat_d00_gt_06.png}
 \includegraphics[height=0.60\linewidth]{figures/ae/car_cccc_gt_00.png}
 \includegraphics[height=0.7\linewidth]{figures/ae/chair_cbc90_gt_00.png}
\caption{Ground truth}
\end{subfigure}
\begin{subfigure}[b]{0.12\linewidth}
\centering
 \includegraphics[height=0.6\linewidth]{figures/ae/boat_cdaff_base_0112.png}
 \includegraphics[height=0.45\linewidth]{figures/ae/avion2_base_d1a810.png}
 %
 \includegraphics[height=0.65\linewidth]{figures/ae/boat_d00_base_0511.png}
 \includegraphics[height=0.60\linewidth]{figures/ae/car_cccc_base_0109.png}
 \includegraphics[height=0.7\linewidth]{figures/ae/chair_cbc90_base_0108.png}
\caption{Pts baseline}
\label{fig:ae_comparison_base}
\end{subfigure}
\begin{subfigure}[b]{0.12\linewidth}
\centering
 \includegraphics[height=0.6\linewidth]{figures/ae/boat_cdaf_psr_02.png}
 \includegraphics[height=0.45\linewidth]{figures/ae/avion2_psr_04.png}
 %
 \includegraphics[height=0.65\linewidth]{figures/ae/boat_d00_psr_03.png}
 \includegraphics[height=0.60\linewidth]{figures/ae/car_psr_01.png}
 \includegraphics[height=0.7\linewidth]{figures/ae/chair_psr_00.png}
\caption{PSR on ours}
\label{fig:ae_comparison_psr}
\end{subfigure}
\begin{subfigure}[b]{0.12\linewidth}
\centering
 \includegraphics[height=0.6\linewidth]{figures/ae/boat_cdaff_sphere_06.png}
 \includegraphics[height=0.45\linewidth]{figures/ae/avion2_sphere_06.png}
 %
 \includegraphics[height=0.65\linewidth]{figures/ae/boat_d00_sphere_00.png}
 \includegraphics[height=0.60\linewidth]{figures/ae/car_cccc_sphere_06.png}
 \includegraphics[height=0.7\linewidth]{figures/ae/chair_cbc90_shpere_06.png}
\caption{Ours sphere}
\end{subfigure}
\begin{subfigure}[b]{0.12\linewidth}
\centering
 \includegraphics[height=0.6\linewidth]{figures/ae/boat_cdaff_1_02.png}
 \includegraphics[height=0.45\linewidth]{figures/ae/avion2_1_02.png}
 %
 \includegraphics[height=0.65\linewidth]{figures/ae/boat_d00_1_04.png}
 \includegraphics[height=0.60\linewidth]{figures/ae/car_cccc_1_02.png}
 \includegraphics[height=0.7\linewidth]{figures/ae/chair_cbc90_1_02.png}
\caption{Ours 1}
\end{subfigure}
\begin{subfigure}[b]{0.12\linewidth}
\centering
 \includegraphics[height=0.6\linewidth]{figures/ae/boat_cdaff_5_03.png}
 \includegraphics[height=0.45\linewidth]{figures/ae/avion2_5_03.png}
%
 \includegraphics[height=0.65\linewidth]{figures/ae/boat_d00_5_03.png}
 \includegraphics[height=0.60\linewidth]{figures/ae/car_cccc_5_03.png}
 \includegraphics[height=0.7\linewidth]{figures/ae/chair_cbc90_5_03.png}
\caption{Ours 5}
\end{subfigure}
\begin{subfigure}[b]{0.12\linewidth}
\centering
 \includegraphics[height=0.6\linewidth]{figures/ae/boat_cdaff_25_04.png}
 \includegraphics[height=0.45\linewidth]{figures/ae/avion2_25_04.png}
 %
 \includegraphics[height=0.65\linewidth]{figures/ae/boat_d00_25_02.png}
 \includegraphics[height=0.60\linewidth]{figures/ae/car_cccc_25_04.png}
 \includegraphics[height=0.7\linewidth]{figures/ae/chair_cbc90_25_04.png}
\caption{Ours 25}
\end{subfigure}
\begin{subfigure}[b]{0.12\linewidth}
\centering
 \includegraphics[height=0.6\linewidth]{figures/ae/boat_cdaff_125_05.png}
 \includegraphics[height=0.45\linewidth]{figures/ae/avion2_125_05.png}
 %
 \includegraphics[height=0.65\linewidth]{figures/ae/boat_d00_125_01.png}
 \includegraphics[height=0.60\linewidth]{figures/ae/car_cccc_125_05.png}
 \includegraphics[height=0.7\linewidth]{figures/ae/chair_cbc90_125_05.png}
\caption{Ours 125}
\end{subfigure}
\caption{
{\bf Auto-encoder.}
We compare the original meshes (a) to meshes obtained by running PSR on the point clouds generated by the baseline (b) and on the densely sampled point cloud from our generated mesh (c),  and to our method generating a surface from a sphere (d), 1 (e), 5 (f), 25 (g), and 125(h) learnable parameterizations. Notice the fine details in (g) and (h) : e.g. the plane's engine and the jib of the ship. %
}
  \label{fig:ae_comparison}
  \vspace{-3mm}

\end{figure*}


\subsection{Auto-encoding 3D shapes}
\label{sec:autoencoding}
%

In this section we evaluate our approach to generate a shape given an input 3D point cloud and compare against the Points baseline.
We evaluate how well our approach can generate the shape, how it can generalize to object categories not seen during training, and its sensitivity to the number of patches.

%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%

%
%

\begin{table}[t!]
\centering
{
  \begin{tabular}{l|c|c}
  \hline
  Method & CD & Metro    \\
%

  \hline
  \hline
%
 Oracle 2500 pts & 0.85 & 1.56 \\
 Oracle 125K pts & - & 1.26 \\
\hline
 Points baseline & {1.91}  & -  \\
 Points baseline + normals & {2.15} & {1.82} (PSR)   \\

 Ours - 1 patch & {1.84} &  {1.53}  \\
 Ours - 1 sphere & {1.72}  & {1.52}  \\
 Ours - 5 patches & {1.57} &  {1.48}  \\
 Ours - 25 patches & {1.56} & {1.47}  \\
 Ours - 125 patches & \textbf{1.51} &  \textbf{1.41}  \\

  \end{tabular}
  }
      \caption{{\bf 3D reconstruction.}
      Comparison of our approach against a point-generation baseline (``CD'' - Chamfer distance, multiplied by $10^3$, computed on 2500 points; ``Metro'' values are multiplied by 10). Note that our approach can be directly evaluated by Metro while the baseline requires performing PSR ~\cite{kazhdan2013screened}. These results can be compared with an Oracle sampling points directly from the ground truth 3D shape followed by PSR (top two rows). See text for details.
      %
      %
      %
      }\label{tab:compare_category}
        \vspace{-3mm}

\end{table}


\myparagraph{Evaluation on surface generation.}
We report quantitative results for shape generation from point clouds in Table~\ref{tab:compare_category}, where each approach is trained over all ShapeNet categories and results are averaged over all categories. 
%
Notice that our approach out-performs the Points baseline on both the Chamfer distance and Metro criteria, even when using a single learned parameterization (patch). %
%
%
%
Also, the Points baseline + normals has worse Chamfer distance than the Points baseline without normals indicating that predicting the normals decreases the quality of the point cloud generation. 
%

We also report performance for two ``oracle'' outputs indicating upper bounds in Table~\ref{tab:compare_category}. 
The first oracle (``Oracle 2500 pts'') randomly samples 2500 points+normals from the ground truth shape and applies PSR. 
The Chamfer distance between the random point set and the ground truth gives an upper bound on performance for point-cloud generation. 
%
%
Notice that our method out-performs the surface generated from the oracle points. 
The second oracle (``Oracle 125K pts'') applies PSR on all 125K points+normals from the ground-truth shape. 
%
It is interesting to note that the Metro distance from this result to the ground truth is not far from the one obtained with our method.

We show qualitative comparisons in Figure~\ref{fig:ae_comparison}.
Notice that the PSR from the baseline point clouds (Figure~\ref{fig:ae_comparison_base}) look noisy and lower quality than the meshes produced directly by our method and PSR performed on points generated from our method as described in Section~\ref{sec:mesh} (Figure~\ref{fig:ae_comparison_psr}). %
%

%
\myparagraph{Sensitivity to number of patches.}
We show in Table~\ref{tab:compare_category} our approach with varying number of learnable parameterizations (patches) in the atlas.
Notice how our approach improves as we increase the number of patches.
Moreover, we also compare with the approach described in Section \ref{sec:mesh} which samples points on the 3D unit sphere instead of 2D patches to obtain a closed mesh. %
Notice that sampling from a sphere quantitatively out-performs a single patch, but multiple patches perform better.
%

We show qualitative results for varying number of learnable parameterizations in Figure~\ref{fig:ae_comparison}. As suggested by the quantitative results, the visual quality improves with the number of parameterizations. 
However, more artifacts appear with more parameterizations, such as close-but-disconnected patches (e.g., sail of the sailboat) . We thus used 25 patches for the single-view reconstruction experiments (Section \ref{sec:svr})



%
%
%
%
%
%
%
%
%
%
%
%
%
%



\begin{table}[t!]
\centering
{
  \begin{tabular}{l|c|c|c|c}
  \hline
  \multicolumn{2}{c|}{Category} & Points  & Ours & Ours   \\
               & &                 baseline &  1 patch &  125 patches  \\
  \hline
  \hline
  \multirow{2}{*}{chair} & LOO &  {3.66} & {3.43} & \textbf{2.69}  \\
   & All &  {1.88} & {1.97}   & \textbf{1.55}\\
     \hline

  \multirow{2}{*}{car} & LOO & {3.38} & {2.96} & \textbf{2.49}   \\
   & All & {1.59} & {2.28} & \textbf{1.56}   \\
     \hline

  \multirow{2}{*}{watercraft} & LOO & {2.90} & {2.61} & \textbf{1.81}   \\
   & All & {1.69} & {1.69} &\textbf{1.23}   \\
     \hline

  \multirow{2}{*}{plane} & LOO & {6.47} & {6.15} & \textbf{3.58} \\
   & All & {1.11} & {1.04} & \textbf{0.86} \\

  \end{tabular} 
 %
 %
 %
 %
 %
 %
 %
 %
 %
 %

 %
  }
  \caption{
  {\bf Generalization across object categories.}
  %
  Comparison of our approach with varying number of patches against the point-generating baseline to generate a specific category when training on all other ShapeNet categories.
  Chamfer distance is reported, multiplied by $10^3$, computed on 2500 points.
  Notice that our approach with 125 patches out-performs all baselines when generalizing to the new category.
  For reference, we also show performance when we train over all categories.
  %
  }\label{tab:gen_category}
    \vspace{-3mm}
\end{table}
\begin{figure}[t!]
\centering
\begin{subfigure}[b]{0.49\linewidth}
\centering
 \includegraphics[width=0.27\linewidth]{figures/gen/cbfa51_gen02.png}
 \includegraphics[width=0.25\linewidth]{figures/gen/cc1b4_gen05.png}
 \includegraphics[width=0.4\linewidth]{figures/gen/cbf18_gen04.png}
\caption{Not trained on chairs}
\end{subfigure}
\vline
\begin{subfigure}[b]{0.49\linewidth}
\centering
 \includegraphics[width=0.28\linewidth]{figures/gen/cbfa51_all01.png}
 \includegraphics[width=0.28\linewidth]{figures/gen/cc1b4_all06.png}
 \includegraphics[width=0.38\linewidth]{figures/gen/cbf18_all03.png}
\caption{Trained on all categories}
\end{subfigure}
\caption{
{\bf Generalization.} (a) Our method (25 patches) can generate surfaces close to a category never seen during training. It, however, has more artifacts than if it has seen the category during training (b), e.g., thin legs and armrests.
}
  \label{fig:gen}
    \vspace{-3mm}
\end{figure}

\myparagraph{Generalization across object categories.} %
%
An important desired property of a shape auto-encoder is that it generalizes well to categories it has not been trained on. To evaluate this, we trained our method on all categories but one target category (``LOO'') for chair, car, watercraft, and plane categories, and evaluated on the held-out category. The corresponding results are reported in Table~\ref{tab:gen_category} and Figure \ref{fig:gen}. We also include performance when the methods are trained on all of the categories including the target category (``All'') for comparison.
Notice that we again out-perform the point-generating baseline on this leave-one-out experiment and that performance improves with more patches. The car category is especially interesting since when trained on all categories the baseline has better results than our method with 1 patch and similar to our method with 125 patches. If not trained on cars, both our approaches clearly outperform the baseline, showing that at least in this case, our approach generalizes better than the baseline. %
The visual comparison shown Figure \ref{fig:gen} gives an intuitive understanding of the consequences of not training for a specific category. When not trained on chairs, our method seems to struggle to define clear thin structures, like legs or armrests, especially when they are associated to a change in the topological genus of the surface. This is expected as these types of structures are not often present in the categories the network was trained on.

%







%
%



%
%
%

\subsection{Single-view reconstruction}
\label{sec:svr}
\captionsetup[table]{skip=4mm}

\begin{table*}[t!]
\centering
{
\small
  \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
   &  pla. &  ben. &  cab. &  car &  cha. &  mon. &  lam. &  spe. &  fir. &  cou. &  tab. &  cel. &  wat. &  mean \\
  \hline
 Ba CD & 2.91 & 4.39 & 6.01 & 4.45 & 7.24 & \textbf{5.95} & 7.42 & 10.4 & 1.83 & \textbf{6.65} & 4.83 & 4.66 & \textbf{4.65} & 5.50 \\
 %
 {PSG CD} & 3.36 & 4.31 & 8.51 & 8.63 & \textbf{6.35} & 6.47 & 7.66 & 15.9 & \textbf{1.58} & 6.92 & \textbf{3.93} & \textbf{3.76} & 5.94 & 6.41  \\
 Ours CD & \textbf{2.54} & \textbf{3.91} & \textbf{5.39} & \textbf{4.18} & 6.77 & {6.71} & \textbf{7.24} & \textbf{8.18} & 1.63 & 6.76 & 4.35 & 3.91 & 4.91 & \textbf{5.11}  \\
 \hline
 \hline
 %
 %
 Ours Metro& 1.31 & 1.89 & 1.80 & 2.04 & 2.11 & 1.68 & 2.81 & 2.39 & 1.57 & 1.78 & 2.28 & 1.03 & 1.84 & 1.89 \\
  \end{tabular}
  }
\medskip
\caption{\textbf{Single-View Reconstruction (per category).} The mean is taken category-wise. The Chamfer Distance reported is computed on 1024 points, after running ICP alignment with the GT point cloud, and multiplied by $10^3$. The Metro distance is multiplied by 10.
  }
  \label{tab:SVR}
  \vspace{1mm}
\end{table*}

\setlength{\belowcaptionskip}{-1pt}


\begin{figure}[t!]

\centering
\begin{subfigure}[b]{0.19\linewidth}
\centering
 \includegraphics[height=0.65\linewidth]{figures/svr/black_background__04copie.png}\\
 \includegraphics[height=0.65\linewidth]{figures/svr/black_background__03copie.png}\\
 \includegraphics[height=0.65\linewidth]{figures/svr/black_background__02copie.png}\\
 \includegraphics[height=0.65\linewidth]{figures/svr/black_background__01copie.png}\\
 \includegraphics[height=0.65\linewidth]{figures/svr/black_background__00copie.png}
\caption{Input}
\end{subfigure}
\begin{subfigure}[b]{0.19\linewidth}
\centering
 \includegraphics[height=0.55\linewidth]{figures/svr/plane1_vox2_01.png}\\[0.1\linewidth]
 ~~~~\includegraphics[height=0.55\linewidth]{figures/svr/lamp_vox_00.png}~~~~\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{figures/svr/chair_vox1_00.png}\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{figures/svr/car2_vox_00.png}\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{figures/svr/car1_vox_01.png}\\[0.05\linewidth]
\caption{{\footnotesize 3D-R2N2}}
\end{subfigure}
\begin{subfigure}[b]{0.19\linewidth}
\centering
 \includegraphics[height=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-christian/white_background_04.png}\\[0.05\linewidth]
 \includegraphics[height=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-christian/white_background_03.png}\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-christian/white_background_02.png}\\[0.1\linewidth]
 ~~~~\includegraphics[height=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-christian/white_background_01.png}~~~~\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-christian/white_background_00.png}\\[0.1\linewidth]
\caption{HSP}
\end{subfigure}
\begin{subfigure}[b]{0.19\linewidth}
\centering
 \includegraphics[height=0.55\linewidth]{figures/svr/plane1_psg2_02.png}\\[0.1\linewidth]
 ~~~~\includegraphics[height=0.65\linewidth]{figures/svr/lamp_psg_00.png}~~~~\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{figures/svr/chair_psg1_00.png}\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{figures/svr/car2_psg_00.png}\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{figures/svr/car1_psg_01.png}\\[0.05\linewidth]
\caption{PSG}
\end{subfigure}
%
%
%
%
%
%
%
%
%
\begin{subfigure}[b]{0.19\linewidth}
\centering
 \includegraphics[height=0.55\linewidth]{figures/svr/plane1_ours2_00.png}\\[0.1\linewidth]
 ~~~~\includegraphics[height=0.55\linewidth]{figures/svr/lamp_ours_00.png}~~~~\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{figures/svr/chair_ours100.png}\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{figures/svr/car2_ours01.png}\\[0.1\linewidth]
 \includegraphics[height=0.55\linewidth]{figures/svr/car1_ours00.png}\\[0.05\linewidth]
\caption{Ours}
\end{subfigure}
\caption{
{\bf Single-view reconstruction comparison.}
From a 2D RGB image (a), 3D-R2N2 \cite{choy20163d} reconstructs a voxel-based 3D model (b),  HSP \cite{Hane:2017} reconstructs a octree-based 3D model (c), PointSetGen \cite{Fan:2017:cvpr} a point cloud based 3D model (d), and our \ournet{} a triangular mesh (e).}
 \label{fig:svr_comparison}
 \vspace{-4mm}
\end{figure}

\begin{figure}[t!]
\centering
\begin{subfigure}[b]{0.30\linewidth}
\begin{minipage}[c]{0.99\linewidth}
\centering
 \includegraphics[height=0.55\linewidth, width=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/png-input/580b57fcd9996e24bc43c26a.png}\\
 \includegraphics[height=0.55\linewidth, width=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/png-input/8-chair-png-image-thumb.png}\\
  \includegraphics[height=0.55\linewidth, width=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/png-input/chair_PNG6885.png}\\
\caption{Input}
\end{minipage}
\end{subfigure}
\begin{subfigure}[b]{0.30\linewidth}
\begin{minipage}[c]{0.99\linewidth}

\centering
 \includegraphics[height=0.55\linewidth, width=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-christian/580b57fcd9996e24bc43c26a.png}\\
 \includegraphics[height=0.55\linewidth, width=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-christian/8-chair.png}\\
  \includegraphics[height=0.55\linewidth, width=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-christian/chair_PNG6885.png}
\caption{HSP}
\end{minipage}

\end{subfigure}
\begin{subfigure}[b]{0.30\linewidth}
\begin{minipage}[c]{0.99\linewidth}

\centering
 \includegraphics[height=0.55\linewidth, width=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-ours/580b57fcd9996e24bc43c26a_input.png}\\
 \includegraphics[height=0.55\linewidth, width=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-ours/8-chair.png}\\
 \includegraphics[height=0.55\linewidth, width=0.55\linewidth]{cvpr2018RebuttalKit/latex/imgs/octree/results-ours/chair-PNG.png}\\

\caption{Ours}
\end{minipage}

\end{subfigure}
\setlength{\belowcaptionskip}{-5pt}
\medskip
\caption{
{\bf Single-view reconstruction comparison on natural images.}
From a 2D RGB image taken from internet (a),  HSP \cite{Hane:2017} reconstructs a octree-based 3D model (b), and our \ournet{} a triangular mesh (c).}
  \label{fig:svr_real_images} \vspace{-4mm}
\end{figure}



We evaluate the potential of our method for single-view reconstruction. We compare qualitatively our results with three state-of-the-art methods, PointSetGen \cite{Fan:2017:cvpr}, 3D-R2N2 \cite{choy20163d} and HSP \cite{Hane:2017} in Figure~\ref{fig:svr_comparison}. To perform the comparison for PointSetGen \cite{Fan:2017:cvpr} and 3D-R2N2 \cite{choy20163d}, we used the trained models made available online by the authors. %
For HSP \cite{Hane:2017}, we asked the authors to run their method on the images in Fig.\ \ref{fig:svr_comparison}. 
Note that since their model was trained on images generated with a different renderer, this comparison is not absolutely fair. To remove the bias we also compared our results with HSP on real images for which none of the methods was trained (Fig.\ \ref{fig:svr_real_images}) which also demonstrates the ability of our network to generalize to real images.


Figure \ref{fig:svr_comparison} emphasizes the importance of the type of output (voxels for 3D-N2D2 and HSP, point cloud for PointSetGen, mesh for us) for the visual appearance of the results. Notice the small details visible on our meshes that may be hard to see on the unstructured point cloud or volumetric representation. Also, it is interesting to see that PointSetGen tends to generate points inside the volume of the 3D shape while our result, by construction, generates points on a surface.


To perform a quantitative comparison against PointSetGen \cite{Fan:2017:cvpr}, we evaluated the Chamfer distance between generated points and points from the original mesh for both PointSetGen and our method with 25 learned parameterizations. However, the PointSetGen network was trained with a translated, rotated, and scaled version of ShapeNet with parameters we did not have access to. We thus first had to align the point clouds resulting from PointSetGen to the ShapeNet models used by our algorithm.
We randomly selected 260 shapes, 20 from each category, and ran the iterative closest point (ICP) algorithm~\cite{besl1992method} to optimize a similarity transform between PointSetGen and the target point cloud. Note that this optimization improves the Chamfer distance between the resulting point clouds, but is not globally convergent. We checked visually that the point clouds from PointSetGen were correctly aligned, and display all alignments on the project webpage\footnote{\url{http://imagine.enpc.fr/~groueixt/atlasnet/PSG.html}.}. To have a fair comparison we ran the same ICP alignment on our results. In Table \ref{tab:SVR} we compared the resulting Chamfer distance. Our method provides the best results on 6 categories whereas PointSetGen and the baseline are best on 4 and 3 categories, respectively. Our method is better on average and generates point clouds of a quality similar to the state of the art. We also report the Metro distance to the original shape, which is the most meaningful measure for our method.

To quantitatively compare against HSP \cite{Hane:2017}, we retrained our method on their publicly available data since train/test splits are different from 3D-R2N2 \cite{choy20163d} and they made their own renderings of ShapeNet data. Results are in Table \ref{tab:hsp_compare}. More details are in the supplementary \cite{appendix}.
\setlength{\belowcaptionskip}{2pt}

\begin{table}[h!]
\centering
%
 \begin{tabular}{l|c|c|c|c|c|c}
 & \multicolumn{1}{|l|}{Chamfer} & \multicolumn{1}{|l|}{Metro} \\
%
%
\hline
HSP  \cite{Hane:2017} & 11.6 &  1.49\\
Ours  (25 patches)  & \textbf{9.52} &  \textbf{1.09} \\
 \end{tabular}
 \medskip
  \caption{{\bf Single-view reconstruction.} Quantitative comparison against HSP \cite{Hane:2017}, a state of the art octree-based method. The average error is reported, on 100 shapes from each category. The Chamfer Distance reported is computed on $10^4$ points, and multiplied by $10^3$. The Metro distance is multiplied by 10. More details are in the supplemetary \cite{appendix}.}\label{tab:hsp_compare}
    \vspace{-3mm}
\end{table}


%
%
%

\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{figures/interpolation/interpolation.png}
\caption{Shape interpolation. \label{fig:interpolation}}
\end{subfigure}
~\vline~
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{figures/correspondences/shape_co-segmentation.pdf}
\caption{Shape correspondences. \label{fig:corresp}}
\end{subfigure}
~\vline~
\begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\linewidth]{figures/param.png}
\caption{Mesh parameterization. \label{fig:mesh_parameterization}}
\end{subfigure}
\caption{{\bf Applications.} Results from three applications of our method. See text for details.
}
\vspace{-10pt}

  \label{fig:applications}
\end{figure*}

\subsection{Additional applications}





\myparagraph{Shape interpolation.}
%
Figure \ref{fig:interpolation} shows shape interpolation.
Each row shows interpolated shapes generated by our \ournet{}, starting from the shape in the first column to the shape in the last. Each intermediate shape is generated using a weighted sum of the latent representations of the two extreme shaped.
Notice how the interpolated shapes gradually add armrests in the first row, and chair legs in the last.

%
%

%
%




%
%
%
%
%
%
%
%
%
%



%
\myparagraph{Finding shape correspondences.}
Figure~\ref{fig:corresp} shows shape correspondences.
We colored the surface of reference chair (left) according to its 3D position.
We transfer the surface colors from the reference shape to the inferred atlas (middle).
Finally, we transfer the atlas colors to other shapes (right) such that points with the same color are parametrized by the same point in the atlas.
Notice that we get semantically meaningful correspondences, such as the chair back, seat, and legs without any supervision from the dataset on semantic information.
%
%

%

%
%
%
%
%
%
%
%
%
%
%
%
%


%
%

\myparagraph{Mesh parameterization}
Most existing rendering pipelines require an atlas for texturing a shape (Figure~\ref{fig:mesh_parameterization}). A good parameterization should minimize
amount of area distortion ($E_a$) and stretch ($E_s$) of a UV map.
%
%
%
We computed average per-triangle distortions for 20 random shapes from each category and found that our inferred atlas usually has relatively high texture distortion ($E_a\!=\!1.9004, E_s\!=\!6.1613$, where undistorted map has $E_a\!=\!E_s\!=\!1$).
Our result, however, is well-suited for distortion minimization because all meshes have disk-like topology and inferred map is bijective, making it easy to further minimize distortion with off-the-shelf geometric optimization~\cite{AQP:2016}, yielding small distortion ($E_a\!=\!1.0016, E_s\!=\!1.025$, see bottom row for example).

%
%
%
%
%
%
%
%
%

%
\myparagraph{Limitations and future work} are detailed in the supplementary materials \cite{appendix}.


==> content/theory.tex <==
\section{Locally parameterized surface generation}

In this section, we detail the theoretical motivation for our approach and present some theoretical guarantees.


%
%
%
\label{sec:theory}
%
We seek to learn to generate a surface of a 3D shape. 
A subset $\mathcal{S}$ of $\mathbb{R}^3$ is a \textit{2-manifold} if, for every point $\mathbf{p}\in\mathcal{S}$, there is an open set $U$ in $\mathbb{R}^2$ and an open set $W$ in $\mathbb{R}^3$ containing $\mathbf{p}$ such that $\mathcal{S}\cap W$ is homeomorphic to $U$. 
The set homeomorphism from $\mathcal{S}\cap W$ to $U$ is called a {\it chart}, and its inverse a {\it parameterization}.
%
A set of charts such that their images cover the 2-manifold is called an {\it atlas} of the 2-manifold. 
The ability to learn an atlas for a 2-manifold would allow a number of applications, such as transfer of a  tessellation to the 2-manifold for meshing and texture mapping (via texture atlases). In this paper, we use the word \textit{surface} in a slightly more generic sense than \textit{2-manifold}, allowing for self-intersections and disjoint sets.

We consider a local parameterization of a 2-manifold and explain how we learn to approximate it. More precisely, let us consider a 2-manifold $\mathcal{S}$, a point  $\mathbf{p}\in\mathcal{S}$ and a parameterization $\varphi$ of $\mathcal{S}$ in a local neighborhood of $\mathbf{p}$. We can assume that $\varphi$ is defined on the open unit square $]0,1[^2$ by first restricting $\varphi$ to an open neighborhood of $\varphi^{-1}(\mathbf{p})$ with disk topology where it is defined (which is possible because $\varphi$ is continuous) and then mapping this neighborhood to the unit square. %

We pose the problem of learning to generate the local 2-manifold previously defined as one of finding a parameterizations $\varphi_{\theta}(x)$ with parameters $\theta$ which map the open unit 2D square $]0,1[^2$ to a good approximation of the desired 2-manifold $\mathcal{S}_{\text{loc}}$. 
Specifically, calling $\mathcal{S}_{\theta}= \varphi_{\theta}(]0,1[^2)$,
we seek to find parameters $\theta$ minimizing the following objective function,
\begin{equation}
    \min_\theta \mathcal{L}\left(\mathcal{S}_{\theta}, \mathcal{S}_{\text{loc}}\right) + \lambda\mathcal{R}\left(\theta\right),
\end{equation}
where $\mathcal{L}$ is a loss over 2-manifolds, $\mathcal{R}$ is a regularization function over parameters $\theta$, and $\lambda$ is a scalar weight. 
In practice, instead of optimizing a loss over 2-manifolds $\mathcal{L}$, we optimize a loss over point sets sampled from these 2-manifolds such as Chamfer and Earth-Mover distance. 
%

%
%
%
%
%
%

One question is, how do we represent the functions $\varphi_{\theta}$? A good family of functions should (i) generate 2-manifolds and (ii) be able to produce a good approximation of the desired 2-manifolds $S_{\text{loc}}$. 
We show that multilayer perceptrons (MLPs) with rectified linear unit (ReLU) nonlinearities almost verify these properties, and thus are an adequate family of functions.
Since it is difficult to design a family of functions that always generate a 2-manifold, we relax this constraint and consider functions that locally generate a 2-manifold. 


\newtheorem{proposition}{Proposition}
%

\begin{proposition}
Let $f$ be a multilayer perceptron with ReLU nonlinearities. There exists a finite set of polygons $P_i$, $i\in \lbrace 1,\ ...,N\rbrace$ such that on each $P_i$ $f$ is an affine function: $\forall x\in P_i, \ f(x)=A_i x+b$, where $A_i$ are $3\times2$ matrices. If for all $i$, $\rank(A_i)=2$, then for any point  $\mathbf{p}$ in the interior of one of the $P_is$ there exists a neighborhood $\mathcal{N}$ of $\mathbf{p}$ such that $f(\mathcal{N})$ is a 2-manifold. 
%
%
%
\end{proposition}

\begin{proof}
The fact that $f$ is locally affine is a direct consequence of the fact that we use ReLU non-linearities. If $\rank(A_i)=2$ the inverse of $A_i x+b$ is well defined on the surface and continuous, thus the image of the interior of each $P_i$ is a 2-manifold.  
%
%
\end{proof}
%

%
To draw analogy to texture atlases in computer graphics, we call the local functions we learn to approximate a 2-manifold {\it learnable parameterizations} and the set of these functions $A$ a {\it learnable atlas}. 
Note that in general, an MLP locally defines a rank 2 affine transformation and thus locally generates a 2-manifold, but may not globally as it may 
%
intersect or overlap with itself. The second reason to choose MLPs as a family is that they can allow us to approximate any continuous surface.

\begin{proposition}
Let $S$ be a 2-manifold that can be parameterized on the unit square. For any $\epsilon>0$ there exists an integer $K$ such that a multilayer perceptron with ReLU non linearities and $K$ hidden units can approximate $S$ with a precision $\epsilon$.
\end{proposition}
%
%
%
%
%
%
%
%
%
%
\vspace*{-13pt}
\begin{proof}
This is a consequence of the universal representation theorem \cite{hornik1991approximation}
\end{proof}
\vspace*{-8pt}

In the next section, we show how to train such MLPs to align with a desired surface. 

%

%
%
%
%
%

%
%
%
%

%

%
%

%
%

%
%
%
%
%
%


%

%
%

%
%
%
%
%



%
%
%

%

%

%

%




